SND@LHC: The Scattering and Neutrino Detector at the LHC

SND@LHC is a compact and stand-alone experiment designed to perform measurements with neutrinos produced at the LHC in the pseudo-rapidity region of ${7.2 < \eta < 8.4}$. The experiment is located 480 m downstream of the ATLAS interaction point, in the TI18 tunnel. The detector is composed of a hybrid system based on an 830 kg target made of tungsten plates, interleaved with emulsion and electronic trackers, also acting as an electromagnetic calorimeter, and followed by a hadronic calorimeter and a muon identification system. The detector is able to distinguish interactions of all three neutrino flavours, which allows probing the physics of heavy flavour production at the LHC in the very forward region. This region is of particular interest for future circular colliders and for very high energy astrophysical neutrino experiments. The detector is also able to search for the scattering of Feebly Interacting Particles. In its first phase, the detector will operate throughout LHC Run 3 and collect a total of 250 $\text{fb}^{-1}$.

==> authorlist_3july2022.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}

%\begin{document}

\centerline{\Large\bf The SND@LHC Collaboration}
\vspace*{1mm}

%\input{authorlist_february2021}

 

%\documentclass{article}
%\usepackage[utf8]{inputenc}

%\begin{document}

%
%\centerline{\Large\bf The SHiP Collaboration}
\vspace*{1mm}
\begin{flushleft}
%-- 
%-- SND@LHC Authorlist as of 1 March 2021
%-- 
G.~Acampora$^{9,c}$, %NAPOLI
C.~Ahdida$^{23}$, %CERN
R.~Albanese$^{9,c,g}$, %NAPOLI
C.~Albrecht$^{25}$, %ZURICH
A.~Alexandrov$^{9,18,20,c}$, %NAPOLI
M.~Andreini$^{23}$, %CERN
A.~Anokhina$^{21,i}$, %SINP
N.~Auberson$^{24}$, %EPFL
C.~Baldanza$^{7}$, %BOLOGNA
C.~Battilana$^{7,b}$, %BOLOGNA
A.~Bay$^{24}$, %EPFL
F.~Bernard$^{24}$, %EPFL
P.~Bestmann$^{23}$, %CERN
C.~Betancourt$^{25}$, %ZURICH
%I.~Bezshyiko$^{25}$, %ZURICH
A.~Blanco$^{29}$,%PORTUGAL
M.~Bogomilov$^{1}$, %SOFIA
D.~Bonacorsi$^{7,b}$, %BOLOGNA
W.M.~Bonivento$^{8}$, %CAGLIARI 
P.~Bordalo$^{29}$, %PORTUGAL
A.~Boyarsky$^{17,d}$, %LEIDEN
G.~Breglio$^{c}$, %NAPOLI
%L.~Buonocore$^{25}$, %ZURICH
A.~Buonaura$^{25}$, %ZURICH
S.~Buontempo$^{9}$, %NAPOLI
V.D.~Cafaro$^{7}$, %BOLOGNA 
M.~Callignon$^{23}$, %CERN 
T.~Camporesi$^{23}$, %CERN
M.~Campanelli$^{28}$, %UCL
V.~Canale$^{9,c}$, %NAPOLI
F.~Cassese$^{9}$, %NAPOLI
A.~Castro$^{7,b}$, %BOLOGNA 
D.~Centanni$^{9,l}$, %NAPOLI
S.A.~Cepeda~Godoy$^{30,31}$, %CHILE
F.~Cerutti$^{23}$, %CERN
N.~Charitonidis$^{23}$, %CERN
M.~Chernyavskiy$^{18}$, %LEBEDEV
K.-Y.~Choi$^{16}$, %KOREA
S.~Cholak$^{24}$, %EPFL
V.~Cicero$^{7,b}$, %BOLOGNA 
F.~Cindolo$^{7}$, %BOLOGNA 
M.~Climescu$^{5}$, %MAINZ
A.P.~Conaboy$^{3}$, %BERLIN
L.~Congedo$^{6,a}$, %BARI
O.~Crespo$^{23}$, %CERN 
M.~Cristinziani$^{4}$, %SIEGEN
A.~Crupano$^{7}$, %BOLOGNA
G.M.~Dallavalle$^{7}$, %BOLOGNA
%A.~Datwyler$^{25}$, %ZURICH
N.~D'Ambrosio$^{10}$, %LNGS
J.~De~Carvalho~Saraiva$^{29}$, %PORTUGAL
P.T.~De~Bryas Dexmiers D'Archiac$^{24}$, %EPFL
G.~De~Lellis$^{9,c,20}$, %NAPOLI
M.~de~Magistris$^{9,l}$,  %NAPOLI
A.~De~Roeck$^{23}$, %CERN
A.~De~Rújula$^{23}$, %CERN
M.~De~Serio$^{6,a}$, %BARI
D.~De~Simone$^{25}$, %ZURICH
L.~Dedenko$^{21}$, %SINP
A.~Di Crescenzo$^{9,c,23}$, %NAPOLI
L.~Di~Giulio$^{23}$, %CERN 
A.~Dolmatov$^{19}$, %KURCHATOV
L.~Dreyfus$^{24}$, %EPFL
O.~Durhan$^{26}$, %ANKARA
F.Fabbri$^{7}$, %BOLOGNA 
D.~Fasanella$^{7,b}$, %BOLOGNA 
F.~Fedotovs$^{28}$, %UCL
M.~Ferrillo$^{25}$, %ZURICH
M.~Ferro-Luzzi$^{23}$, %CERN
F.~Fienga$^{c}$, %NAPOLI
R.A.~Fini$^{6}$, %BARI
A.~Fiorillo$^{9,c}$, %NAPOLI
P.~Fonte$^{29}$,%PORTUGAL
R.~Fresa$^{9,c}$, %NAPOLI
R.~Frei$^{24}$, %EPFL
W.~Funk$^{23}$, %CERN
G.~Galati$^{6,a}$, %BARI
V.~Galkin$^{21,i}$, %SINP 
F.~Garay~Walls$^{30,32}$, %CHILE
R.~Garcia~Alia$^{23}$, %CERN 
%V.~Gentile$^{9,20,c}$, %NAPOLI
A.~Gerbershagen$^{23}$, %CERN
V.~Giordano$^{7}$, %BOLOGNA 
A.~Golovatiuk$^{9,c}$, %NAPOLI
A.~Golutvin$^{27,20}$, %IMPERIAL 
M.~Gorshenkov$^{20}$, %MISIS
E.~Graverini$^{24}$, %EPFL
J.-L.~Grenard$^{23}$, %CERN 
A.M.~Guler$^{26}$, %ANKARA
V.~Gulyaeva$^{21,i}$, %SINP
G.J.~Haefeli$^{24}$, %EPFL
J.C.~Helo$^{30,33}$, %CHILE
E.van~Herwijnen$^{20}$, %MISiS
P.~Iengo$^{9}$, %NAPOLI
S.~Ilieva$^{1},$ %SOFIA
A.~Infantino$^{23}$, %CERN 
A.~Irace$^{c}$, %NAPOLI
A.~Iuliano$^{9,c}$, %NAPOLI
R.~Jacobsson$^{23}$, %CERN
M.~Jacquart$^{24}$, %EPFL
C.~Kamiscioglu$^{26,f}$, %ANKARA
E.~Khalikov$^{21}$, %SINP
Y.G.~Kim$^{14}$, %KOREA
S.H.~Kim$^{13}$, %KOREA
M.~Komatsu$^{11}$, %NAGOYA
N.~Konovalova$^{18,20}$, %LEBEDEV
S.~Kovalenko$^{30,31}$, %CHILE
I.~Krasilnikova$^{20}$, %MISIS
S.~Kuleshov$^{30,31}$, %CHILE
H.M.~Lacker$^{3}$, %BERLIN
O.~Lantwin$^{20}$, %ZURICH, now at ANNECY
F.~Lasagni~Manghi$^{7}$, %BOLOGNA 
A.~Lauria$^{9,c}$, %NAPOLI
K.S.~Lee$^{15}$, %KOREA 
K.Y.~Lee$^{13}$, %KOREA
N.~Leonardo$^{29}$, %PORTUGAL
M.P.~Liz~Vargas$^{30,31}$, %CHILE 
S.~Lo Meo$^{7,k}$, %BOLOGNA 
C.~Lemettais$^{24}$, %EPFL
V.P.~Loschiavo$^{9,g}$,  %NAPOLI
L.~Lopes$^{29}$, %PORTUGAL
B.~Lussi$^{25}$, %ZURICH
S.~Marcellini$^{7}$, %BOLOGNA 
A.~Margiotta$^{7,b}$, %BOLOGNA 
A.~Magnan$^{27}$, %IMPERIAL
R.~Maier$^{25}$, %ZURICH
M.~Maietta$^{23}$, %CERN 
A.~Malinin$^{19}$, %KURCHATOV
V.R.~Marrazzo$^{c}$, %NAPOLI
Y.~Maurer$^{23}$, %CERN 
A.K.~Managadze$^{21}$, %SINP
A.~Mascellani$^{24}$, %EPFL
A.~Miano$^{9,c}$,  %NAPOLI
A.~Mikulenko$^{17}$, %LEIDEN
F.~Minelli$^{24}$, %EPFL
A.~Montanari$^{7}$, %BOLOGNA 
M.C.~Montesi$^{9,c}$, %NAPOLI
T.~Naka$^{12}$, %TOHO
F.L.~Navarria$^{7}$, %BOLOGNA
S.~Ogawa$^{12}$, %TOHO
N.~Okateva$^{18,20}$, %LEBEDEV
N.~Owtscharenko$^{4}$, %SIEGEN
%P.H.~Owen$^{25}$, %ZURICH
M.~Ovchynnikov$^{17}$, %LEIDEN
B.D.~Park$^{13}$, %KOREA
G.~Passeggio$^{9}$, %NAPOLI
A.~Pastore$^{6}$, %BARI
M.~Patel$^{27,20}$, %IMPERIAL
L.~Patrizii$^{7}$, %BOLOGNA 
A.~Perrotta$^{7}$, %BOLOGNA
A.~Petrov$^{19}$, %KURCHATOV
D.~Podgrudkov$^{21,i}$, %SINP
A.~Polini$^{7}$, %BOLOGNA 
N.~Polukhina$^{18,20,e}$, %LEBEDEV
A.~Prota$^{9,c}$, %NAPOLI
F.~Queiroz$^{34}$, %BRAZIL
A.~Quercia$^{9,c}$, %NAPOLI
S.~Ramos$^{29}$, %PORTUGAL
F.~Ratnikov$^{22}$, %YANDEX
A.~Reghunath$^{3}$, %BERLIN
M.~Riccio$^{c}$, %NAPOLI
A.B.~Rodrigues~Cavalcante$^{24}$, %EPFL
T.~Roganova$^{21,i}$, %SINP
T.~Rovelli$^{7,b}$, %BOLOGNA 
O.~Ruchayskiy$^{2}$, %COPENHAGEN
T.~Ruf$^{23}$, %CERN
M.~Sabate~Gilarte$^{23}$, %CERN
F.~Sanchez~Galan$^{23}$, %CERN
P.~Santos~Diaz$^{23}$, %CERN
M.~Schaffner$^{25}$, %ZURICH
O.~Schneider$^{24}$,  %EPFL
G.~Sekhniaidze$^{9}$, %NAPOLI
N.~Serra$^{25}$, %ZURICH
T.~Shchedrina$^{18,20}$, %LEBEDEV
L.~Shchutska$^{24}$, %EPFL
V.~Shevchenko$^{19,20}$,  %KURCHATOV
H.~Shibuya$^{12,h}$, %TOHO
S.~Shirobokov$^{27}$, %IMPERIAL
E.~Shmanin$^{20}$, %MISIS
S.~Simone$^{6,a}$, %BARI
G.P.~Siroli$^{7,b}$, %BOLOGNA 
L.~Sito$^{c}$, %NAPOLI
G.~Sirri$^{7,b}$, %BOLOGNA
J.~Schmidt$^{3}$, %BERLIN
G.~Soares$^{29}$,%PORTUGAL //no email
J.Y.~Sohn$^{13}$, %KOREA
O.J.~Soto~Sandoval$^{30,33}$, %CHILE
M.~Spurio$^{7,b}$, %BOLOGNA 
N.~Starkov$^{18,20}$, %LEBEDEV
J.L.~Tastet$^{2}$, %COPENHAGEN
I.~Timiryasov$^{2}$, %NBI
V.~Tioukov$^{9}$, %NAPOLI
N.~Tosi$^{7}$, %BOLOGNA 
C.~Trippl$^{24}$, %EPFL
%F.~Tramontano$^{9,c}$, %NAPOLI
P.A.~Ulloa~Poblete$^{30,33}$, %CHILE
E.~Ursov$^{21,i}$, %SINP
A.~Ustyuzhanin$^{9,22}$, %NAPOLI
G.~Vankova-Kirilova$^{1}$, %SOFIA
C.~Vendeuvre$^{23}$, %CERN
C.~Visone$^{9,c}$,  %NAPOLI
A.~Vollhardt$^{25}$, %ZURICH
R.~Wanke$^{5}$, %MAINZ
C.S.~Yoon$^{13}$, %KOREA
J.~Zamora~Saa$^{30,31}$, %CHILE
E.~Zaffaroni$^{24}$, %EPFL 
H.J.~Zick$^{3}$ %BERLIN
\vspace*{1cm}

{\footnotesize \it

$ ^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$ ^{2}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$ ^{3}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$ ^{4}$Department Physik, Universit\"{a}t Siegen, Siegen, Germany\\
$ ^{5}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$ ^{6}$Sezione INFN di Bari, Bari, Italy\\
$ ^{7}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{8}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{9}$Sezione INFN di Napoli, Napoli, Italy\\
$ ^{10}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$ ^{11}$Nagoya University, Nagoya, Japan\\
$ ^{12}$Toho University, Funabashi, Chiba, Japan\\
$ ^{13}$Department of Physics Education and RINS, Gyeongsang National University, Jinju, Korea\\
$ ^{14}$Gwangju National University of Education, Gwangju, Korea\\
$ ^{15}$Korea University, Seoul, Korea\\
$ ^{16}$Sungkyunkwan University, Suwon-si, Gyeong Gi-do, Korea\\
$ ^{17}$University of Leiden, Leiden, The Netherlands\\
$ ^{18}$P.N.~Lebedev Physical Institute (LPI RAS), Moscow, Russia\\
$ ^{19}$National Research Centre 'Kurchatov Institute', Moscow, Russia\\
$ ^{20}$National University of Science and Technology 'MISiS', Moscow, Russia\\
$ ^{21}$Skobeltsyn Institute of Nuclear Physics of Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{22}$National Research University Higher School of Economics, Moscow, Russia \\
%Yandex School of Data Analysis, Moscow, Russia\\
$ ^{23}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{24}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{25}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$ ^{26}$Middle East Technical University (METU), Ankara, Turkey\\
$ ^{27}$Imperial College London, London, United Kingdom\\
$ ^{28}$University College London, London, United Kingdom\\
$ ^{29}$Laboratory of Instrumentation and Experimental Particle Physics (LIP), Lisbon, Portugal\\
$ ^{30}$Millennium Institute for Subatomic physics at high energy frontier-SAPHIR, Fernandez Concha 700, Santiago, Chile \\
$ ^{31}$Center for Theoretical and Experimental Particle Physics, Facultad de Ciencias Exactas, Universidad Andrés Bello, Fernandez Concha 700, Santiago, Chile$ ^{j}$ \\
$ ^{32}$Pontificia Universidad Católica de Chile, Santiago, Chile$ ^{j}$\\
$ ^{33}$Departamento de Física, Facultad de Ciencias, Universidad de La Serena, Avenida Cisternas 1200, La Serena, Chile$ ^{j}$\\
$ ^{34}$International Institute of Physics at the Federal University of Rio Grande do Norte, Rio Grande do Norte, Brazil\\
$ ^{a}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{c}$Universit\`{a} di Napoli ``Federico II'', Napoli, Italy\\
$ ^{d}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$ ^{e}$National Research Nuclear University (MEPhI), Moscow, Russia\\
$ ^{f}$Ankara University, Ankara, Turkey\\
$ ^{g}$Consorzio CREATE, Napoli, Italy\\
$ ^{h}$Present address: Faculty of Engineering, Kanagawa University, Yokohama, Japan\\
$ ^{i}$Also at: Lomonosov Moscow State University, Faculty of Physics, Moscow, Russia\\
$ ^{j}$Associated to: Millennium Institute for Subatomic physics at high energy frontier-SAPHIR, Fernandez Concha 700, Santiago, Chile \\
%$ ^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
%$ ^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
%$ ^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
%$ ^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
$ ^{k}$ENEA Research Centre E. Clementel, Bologna, Italy\\
$ ^{l}$Universit\`{a} di Napoli Parthenope, Napoli, Italy\\
$ ^{m}$Universit\`{a} del Sannio, Benevento, Italy\\
}
\end{flushleft}

==> authorlist_5may2022.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}

%\begin{document}

\centerline{\Large\bf The SND@LHC Collaboration}
\vspace*{1mm}

%\input{authorlist_february2021}

 

%\documentclass{article}
%\usepackage[utf8]{inputenc}

%\begin{document}

%
%\centerline{\Large\bf The SHiP Collaboration}
\vspace*{1mm}
\begin{flushleft}
%-- 
%-- SND@LHC Authorlist as of 1 March 2021
%-- 
G.~Acampora$^{9,c}$, %NAPOLI
C.~Ahdida$^{23}$, %CERN
R.~Albanese$^{9,c,g}$, %NAPOLI
C.~Albrecht$^{25}$, %ZURICH
A.~Alexandrov$^{9,18,20,c}$, %NAPOLI
M.~Andreini$^{23}$, %CERN
A.~Anokhina$^{21,i}$, %SINP
N.~Auberson$^{24}$, %EPFL
C.~Baldanza$^{7}$, %BOLOGNA
C.~Battilana$^{7,b}$, %BOLOGNA
A.~Bay$^{24}$, %EPFL
F.~Bernard$^{24}$, %EPFL
P.~Bestmann$^{23}$, %CERN
C.~Betancourt$^{25}$, %ZURICH
%I.~Bezshyiko$^{25}$, %ZURICH
A.~Blanco$^{29}$,%PORTUGAL
M.~Bogomilov$^{1}$, %SOFIA
D.~Bonacorsi$^{7,b}$, %BOLOGNA
W.M.~Bonivento$^{8}$, %CAGLIARI 
P.~Bordalo$^{29}$, %PORTUGAL
A.~Boyarsky$^{17,d}$, %LEIDEN
G.~Breglio$^{c}$, %NAPOLI
%L.~Buonocore$^{25}$, %ZURICH
A.~Buonaura$^{25}$, %ZURICH
S.~Buontempo$^{9}$, %NAPOLI
V.D.~Cafaro$^{7}$, %BOLOGNA 
M.~Callignon$^{23}$, %CERN 
T.~Camporesi$^{23}$, %CERN
M.~Campanelli$^{28}$, %UCL
V.~Canale$^{9,c}$, %NAPOLI
F.~Cassese$^{9}$, %NAPOLI
D.~Centanni$^{9,l}$, %NAPOLI
S.A.~Cepeda~Godoy$^{30,31}$, %CHILE
F.~Cerutti$^{23}$, %CERN
N.~Charitonidis$^{23}$, %CERN
M.~Chernyavskiy$^{18}$, %LEBEDEV
K.-Y.~Choi$^{16}$, %KOREA
S.~Cholak$^{24}$, %EPFL
V.~Cicero$^{7,b}$, %BOLOGNA 
V.~Cindolo$^{7}$, %BOLOGNA 
M.~Climescu$^{5}$, %MAINZ
A.P.~Conaboy$^{3}$, %BERLIN
L.~Congedo$^{6,a}$, %BARI
O.~Crespo$^{23}$, %CERN 
M.~Cristinziani$^{4}$, %SIEGEN
A.~Crupano$^{7}$, %BOLOGNA
G.M.~Dallavalle$^{7}$, %BOLOGNA
%A.~Datwyler$^{25}$, %ZURICH
N.~D'Ambrosio$^{10}$, %LNGS
J.~De~Carvalho~Saraiva$^{29}$, %PORTUGAL
P.T.~De~Bryas Dexmiers D'Archiac$^{24}$, %EPFL
G.~De~Lellis$^{9,c,20}$, %NAPOLI
M.~de~Magistris$^{9,l}$,  %NAPOLI
A.~De~Roeck$^{23}$, %CERN
A.~De~Rujula$^{23}$, %CERN
M.~De~Serio$^{6,a}$, %BARI
D.~De~Simone$^{25}$, %ZURICH
L.~Dedenko$^{21}$, %SINP
A.~Di Crescenzo$^{9,c,23}$, %NAPOLI
L.~Di~Giulio$^{23}$, %CERN 
A.~Dolmatov$^{19}$, %KURCHATOV
L.~Dreyfus$^{24}$, %EPFL
O.~Durhan$^{26}$, %ANKARA
F.Fabbri$^{7}$, %BOLOGNA 
D.~Fasanella$^{7,b}$, %BOLOGNA 
F.~Fedotovs$^{28}$, %UCL
M.~Ferrillo$^{25}$, %ZURICH
M.~Ferro-Luzzi$^{23}$, %CERN
F.~Fienga$^{c}$, %NAPOLI
R.A.~Fini$^{6}$, %BARI
A.~Fiorillo$^{9,c}$, %NAPOLI
P.~Fonte$^{29}$,%PORTUGAL
R.~Fresa$^{9,c}$, %NAPOLI
R.~Frei$^{24}$, %EPFL
W.~Funk$^{23}$, %CERN
G.~Galati$^{6,a}$, %BARI
V.~Galkin$^{21,i}$, %SINP 
F.~Garay~Walls$^{30,32}$, %CHILE
R.~Garcia~Alia$^{23}$, %CERN 
%V.~Gentile$^{9,20,c}$, %NAPOLI
A.~Gerbershagen$^{23}$, %CERN
V.~Giordano$^{7}$, %BOLOGNA 
A.~Golovatiuk$^{9,c}$, %NAPOLI
A.~Golutvin$^{27,20}$, %IMPERIAL 
M.~Gorshenkov$^{20}$, %MISIS
E.~Graverini$^{24}$, %EPFL
J.-L.~Grenard$^{23}$, %CERN 
A.M.~Guler$^{26}$, %ANKARA
V.~Gulyaeva$^{21,i}$, %SINP
G.J.~Haefeli$^{24}$, %EPFL
J.C.~Helo$^{30,33}$, %CHILE
E.van~Herwijnen$^{20}$, %MISiS
P.~Iengo$^{9}$, %NAPOLI
S.~Ilieva$^{1},$ %SOFIA
A.~Infantino$^{23}$, %CERN 
A.~Irace$^{c}$, %NAPOLI
A.~Iuliano$^{9,c}$, %NAPOLI
R.~Jacobsson$^{23}$, %CERN
M.~Jacquart$^{24}$, %EPFL
C.~Kamiscioglu$^{26,f}$, %ANKARA
E.~Khalikov$^{21}$, %SINP
Y.G.~Kim$^{14}$, %KOREA
S.H.~Kim$^{13}$, %KOREA
M.~Komatsu$^{11}$, %NAGOYA
N.~Konovalova$^{18,20}$, %LEBEDEV
S.~Kovalenko$^{30,31}$, %CHILE
I.~Krasilnikova$^{20}$, %MISIS
S.~Kuleshov$^{30,31}$, %CHILE
H.M.~Lacker$^{3}$, %BERLIN
O.~Lantwin$^{20}$, %ZURICH, now at ANNECY
F.~Lasagni~Manghi$^{7}$, %BOLOGNA 
A.~Lauria$^{9,c}$, %NAPOLI
K.S.~Lee$^{15}$, %KOREA 
K.Y.~Lee$^{13}$, %KOREA
N.~Leonardo$^{29}$, %PORTUGAL
M.P.~Liz~Vargas$^{30,31}$, %CHILE 
S.~Lo Meo$^{7,k}$, %BOLOGNA 
C.~Lemettais$^{24}$, %EPFL
V.P.~Loschiavo$^{9,g}$,  %NAPOLI
L.~Lopes$^{29}$, %PORTUGAL
B.~Lussi$^{25}$, %ZURICH
S.~Marcellini$^{7}$, %BOLOGNA 
A.~Margiotta$^{7,b}$, %BOLOGNA 
A.~Magnan$^{27}$, %IMPERIAL
R.~Maier$^{25}$, %ZURICH
M.~Maietta$^{23}$, %CERN 
A.~Malinin$^{19}$, %KURCHATOV
V.R.~Marrazzo$^{c}$, %NAPOLI
Y.~Maurer$^{23}$, %CERN 
A.K.~Managadze$^{21}$, %SINP
A.~Mascellani$^{24}$, %EPFL
A.~Miano$^{9,c}$,  %NAPOLI
A.~Mikulenko$^{17}$, %LEIDEN
F.~Minelli$^{24}$, %EPFL
A.~Montanari$^{7}$, %BOLOGNA 
M.C.~Montesi$^{9,c}$, %NAPOLI
T.~Naka$^{12}$, %TOHO
F.L.~Navarria$^{7}$, %BOLOGNA
S.~Ogawa$^{12}$, %TOHO
N.~Okateva$^{18,20}$, %LEBEDEV
N.~Owtscharenko$^{4}$, %SIEGEN
%P.H.~Owen$^{25}$, %ZURICH
M.~Ovchynnikov$^{17}$, %LEIDEN
B.D.~Park$^{13}$, %KOREA
G.~Passeggio$^{9}$, %NAPOLI
A.~Pastore$^{6}$, %BARI
M.~Patel$^{27,20}$, %IMPERIAL
L.~Patrizii$^{7}$, %BOLOGNA 
A.~Perrotta$^{7}$, %BOLOGNA
A.~Petrov$^{19}$, %KURCHATOV
D.~Podgrudkov$^{21,i}$, %SINP
A.~Polini$^{7}$, %BOLOGNA 
N.~Polukhina$^{18,20,e}$, %LEBEDEV
A.~Prota$^{9,c}$, %NAPOLI
F.~Queiroz$^{34}$, %BRAZIL
A.~Quercia$^{9,c}$, %NAPOLI
S.~Ramos$^{29}$, %PORTUGAL
F.~Ratnikov$^{22}$, %YANDEX
A.~Reghunath$^{3}$, %BERLIN
M.~Riccio$^{c}$, %NAPOLI
A.B.~Rodrigues~Cavalcante$^{24}$, %EPFL
T.~Roganova$^{21,i}$, %SINP
T.~Rovelli$^{7,b}$, %BOLOGNA 
O.~Ruchayskiy$^{2}$, %COPENHAGEN
T.~Ruf$^{23}$, %CERN
M.~Sabate~Gilarte$^{23}$, %CERN
F.~Sanchez~Galan$^{23}$, %CERN
P.~Santos~Diaz$^{23}$, %CERN
M.~Schaffner$^{25}$, %ZURICH
O.~Schneider$^{24}$,  %EPFL
G.~Sekhniaidze$^{9}$, %NAPOLI
N.~Serra$^{25}$, %ZURICH
T.~Shchedrina$^{18,20}$, %LEBEDEV
L.~Shchutska$^{24}$, %EPFL
V.~Shevchenko$^{19,20}$,  %KURCHATOV
H.~Shibuya$^{12,h}$, %TOHO
S.~Shirobokov$^{27}$, %IMPERIAL
E.~Shmanin$^{20}$, %MISIS
S.~Simone$^{6,a}$, %BARI
G.P.~Siroli$^{7,b}$, %BOLOGNA 
L.~Sito$^{c}$, %NAPOLI
G.~Sirri$^{7,b}$, %BOLOGNA
J.~Schmidt$^{3}$, %BERLIN
G.~Soares$^{29}$,%PORTUGAL //no email
J.Y.~Sohn$^{13}$, %KOREA
O.J.~Soto~Sandoval$^{30,33}$, %CHILE
M.~Spurio$^{7,b}$, %BOLOGNA 
N.~Starkov$^{18,20}$, %LEBEDEV
J.L.~Tastet$^{2}$, %COPENHAGEN
I.~Timiryasov$^{2}$, %NBI
V.~Tioukov$^{9}$, %NAPOLI
N.~Tosi$^{7}$, %BOLOGNA 
C.~Trippl$^{24}$, %EPFL
%F.~Tramontano$^{9,c}$, %NAPOLI
P.A.~Ulloa~Poblete$^{30,33}$, %CHILE
E.~Ursov$^{21,i}$, %SINP
A.~Ustyuzhanin$^{9,22}$, %NAPOLI
G.~Vankova-Kirilova$^{1}$, %SOFIA
C.~Vendeuvre$^{23}$, %CERN
C.~Visone$^{9,c}$,  %NAPOLI
A.~Vollhardt$^{25}$, %ZURICH
R.~Wanke$^{5}$, %MAINZ
C.S.~Yoon$^{13}$, %KOREA
J.~Zamora~Saa$^{30,31}$, %CHILE
E.~Zaffaroni$^{24}$, %EPFL 
H.J.~Zick$^{3}$ %BERLIN
\vspace*{1cm}

{\footnotesize \it

$ ^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$ ^{2}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$ ^{3}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$ ^{4}$Department Physik, Universit\"{a}t Siegen, Siegen, Germany\\
$ ^{5}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$ ^{6}$Sezione INFN di Bari, Bari, Italy\\
$ ^{7}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{8}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{9}$Sezione INFN di Napoli, Napoli, Italy\\
$ ^{10}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$ ^{11}$Nagoya University, Nagoya, Japan\\
$ ^{12}$Toho University, Funabashi, Chiba, Japan\\
$ ^{13}$Department of Physics Education and RINS, Gyeongsang National University, Jinju, Korea\\
$ ^{14}$Gwangju National University of Education, Gwangju, Korea\\
$ ^{15}$Korea University, Seoul, Korea\\
$ ^{16}$Sungkyunkwan University, Suwon-si, Gyeong Gi-do, Korea\\
$ ^{17}$University of Leiden, Leiden, The Netherlands\\
$ ^{18}$P.N.~Lebedev Physical Institute (LPI RAS), Moscow, Russia\\
$ ^{19}$National Research Centre 'Kurchatov Institute', Moscow, Russia\\
$ ^{20}$National University of Science and Technology 'MISiS', Moscow, Russia\\
$ ^{21}$Skobeltsyn Institute of Nuclear Physics of Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{22}$National Research University Higher School of Economics, Moscow, Russia \\
%Yandex School of Data Analysis, Moscow, Russia\\
$ ^{23}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{24}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{25}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$ ^{26}$Middle East Technical University (METU), Ankara, Turkey\\
$ ^{27}$Imperial College London, London, United Kingdom\\
$ ^{28}$University College London, London, United Kingdom\\
$ ^{29}$Laboratory of Instrumentation and Experimental Particle Physics (LIP), Lisbon, Portugal\\
$ ^{30}$Millennium Institute for Subatomic physics at high energy frontier-SAPHIR, Fernandez Concha 700, Santiago, Chile \\
$ ^{31}$Center for Theoretical and Experimental Particle Physics, Facultad de Ciencias Exactas, Universidad Andrés Bello, Fernandez Concha 700, Santiago, Chile$ ^{j}$ \\
$ ^{32}$Pontificia Universidad Católica de Chile, Santiago, Chile$ ^{j}$\\
$ ^{33}$Departamento de Física, Facultad de Ciencias, Universidad de La Serena, Avenida Cisternas 1200, La Serena, Chile$ ^{j}$\\
$ ^{34}$International Institute of Physics at the Federal University of Rio Grande do Norte, Rio Grande do Norte, Brazil\\
$ ^{a}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{c}$Universit\`{a} di Napoli ``Federico II'', Napoli, Italy\\
$ ^{d}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$ ^{e}$National Research Nuclear University (MEPhI), Moscow, Russia\\
$ ^{f}$Ankara University, Ankara, Turkey\\
$ ^{g}$Consorzio CREATE, Napoli, Italy\\
$ ^{h}$Present address: Faculty of Engineering, Kanagawa University, Yokohama, Japan\\
$ ^{i}$Also at: Lomonosov Moscow State University, Faculty of Physics, Moscow, Russia\\
$ ^{j}$Associated to: Millennium Institute for Subatomic physics at high energy frontier-SAPHIR, Fernandez Concha 700, Santiago, Chile \\
%$ ^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
%$ ^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
%$ ^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
%$ ^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
$ ^{k}$ENEA Research Centre E. Clementel, Bologna, Italy\\
$ ^{l}$Universit\`{a} di Napoli Parthenope, Napoli, Italy\\
$ ^{m}$Universit\`{a} del Sannio, Benevento, Italy\\
}
\end{flushleft}


%\end{document}



%\end{document}


==> sections/Internal_comments.tex <==
Chris:
1. The calibration procedure for the scifi, veto and muon system should be described in the DAQ section. -> Agree (Ettore)

2. Description of the gain should be included in the DAQ section, or else a small statement and reference. -> Agree (Ettore)

Regardng 1 and 2, I described the calibration briefly and mentioned that the QDC has the variable gain, I would not go in too many details here, but let me know if I should be more specific in some parts (Ettore)

3. British or American English? -> British (Ettore)

4. Need consistent way to introduce dimensions, i.e. "bars with dimensions 1 x 6 x 82.5 cm^3" or with "()" -> \SI[product-units=power]{1 x 6 x 82.5}{cm}, no parentheses (careful, the unit is automatic raised to the correct power, so put cm) (Ettore)

5. How to introduce figures. Should it be "Figure #", "Fig. #", "figure #" or "fig. #"? -> Figure~\ref{...} (Ettore)

6. Need someone to check acronyms. Specifically need to make sure first instance of SiPM or FE is properly carried through and the acronym is not defined more than once. -> Yes, this will be done later, now you can assume someone already defined those in your sections (Ettore)

7. Consistent style or references needed. -> What do you mean here? the style is defined in JHEP.bst, then you just need to add the references in references.bib.

8. 


==> sections/daq_old.tex <==

\section{The Data Acquisition and Online systems}
\label{sec:daq}
As discussed in Sections~\ref{sec:veto}, \ref{sec:scifi} and~\ref{sec:muon}, the SND@LHC detector features two types of electronic sub-systems:
\begin{itemize}
    \item Scintillator bars read out by SiPMs, used for the Veto, the hadronic calorimeter and  muon system;
    \item Scintillating fibres read out by SiPMs, used for the Target Tracker.
\end{itemize}

These sub-systems are read out with the same Data Acquisition (DAQ) electronics, based on a main DAQ board, featuring a Cyclone V FPGA, and four front-end (FE) boards, based on the TOFPET2 ASIC, by PETsys~\cite{tofpet2_url}.

The detector uses a total of 37 DAQ boards, which run synchronously with the LHC bunch crossing clock.
It is operated in a trigger-less fashion, i.e.\ all hits recorded by each board are transmitted to the DAQ server.
Noise reduction is performed at the front-end level by setting an appropriate threshold for each channel or disabling noisy channels, and on the DAQ server, after event building.

\subsection{DAQ architecture}
\label{subsec:daq-structure}

The DAQ system of the SND@LHC detector is composed of:
\begin{itemize}
    \item 37 DAQ boards, with four FE boards each, described in Section~\ref{subsec:daq-electronics}. They read out the signals from the SiPMs, digitize them and send recorded data to a server.
    \item One Trigger Timing Control (TTC) crate, described in Section~\ref{subsec:lhc-signals}, to receive the LHC clock and orbit signals from the Beam Synchronous Timing (BST) system and transmit them to the DAQ boards. This is necessary to have them run synchronously with the LHC bunch crossing.
    \item Two servers, located on the surface: one receives data from the DAQ boards and combines it into events, as described in Section~\ref{subsec:daq-events}, which are then saved to disk; the other controls all aspects of the DAQ and performs data quality monitoring.
\end{itemize}
Details about each component are given in the following sections. A schematic representation of the DAQ system is shown in Figure~\ref{fig:daq-scheme}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{images/daq/snd-daq-scheme.pdf}
    \caption{Simplified scheme of the SND@LHC DAQ system.}
    \label{fig:daq-scheme}
\end{figure}

\subsection{DAQ electronics}
\label{subsec:daq-electronics}

The DAQ board, shown in Figure~\ref{fig:daq-board}, is based on the Mercury SA1 module from Enclustra~\cite{enclustra_mercury_sa1}, featuring an Altera Cyclone~V FPGA. The main characteristics of this board are:
\begin{itemize}
    \item four high-speed connectors for the FE boards;
    \item TTCrx ASIC~\cite{ttc_web} with an optical fibre receiver, used to receive the clock and synchronous signals from the TTC system;
    \item \SI{1}{Gb} Ethernet port, used for data and command transmission;
    \item LEMO connector to deliver the bias voltage to SiPMs.
\end{itemize}

Each DAQ board collects the data digitized by FE boards and transmits it to the DAQ server, running on a PC on the surface.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/daq/daq_board.jpg}
    \caption{The DAQ board. The four FE board connectors are visible on the left, the TTCrx and optical receiver on the bottom-right, the Enclustra Mercury SA 1 module in the centre.}
    \label{fig:daq-board}
\end{figure}

The FE board, shown in Figure~\ref{fig:fe-board}, contains two TOFPET2 ASICs, used to read out the SiPMs, and has temperature monitoring capabilities of both the SiPMs and the board itself.
Each TOFPET2 ASIC can read out \num{64} channels, for a total of \num{128} channels per FE board and \num{512} per DAQ board.
The TOFPET2 records all the hits that exceed a predefined threshold and provides energy and timestamp information.
More details are given in the following section.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/daq/TOFPET.jpg}
    \caption{The FE board. The two TOFPET2 ASICS (centre) and the SiPM connectors (left) are visible.}
    \label{fig:fe-board}
\end{figure}

\subsection{The TOFPET2 ASIC}
\label{subsec:tofpet}
The TOFPET2 is a 64-channels readout and digitization ASIC, designed for time of flight positron emission tomography systems ~\cite{tofpet2_datasheet}.
It integrates signal amplification circuitry, discriminators, charge integrators, Analog to Digital converters (ADC, also indicated as QDCs, charge to digital converters) and Time to Digital converters (TDC).
It allows to measure signals produced by SiPMs and to record their timestamp and charge.

Each channel features a preamplifier and two amplifiers, one optimized for time resolution and the second for charge integration.
A combination of up to three discriminators with configurable thresholds can be used: the first one (identified with T1) is mainly used for timing measurements, and it is normally the lowest threshold one, while the other two (T2 and E) are used to reject low amplitude pulses and start charge integration.
TDCs feature a time binning of \SI{\sim 40}{ps} and  QDCs have a linear response up to \SI{1500}{pC} input charge.
In addition, the gain of the QDC branch can be selected to have a value between \num{1.00} and \num{3.65}, to achieve the best resolution and dynamic range, depending on the signal generated by the SiPMs~\cite{tofpet2_datasheet}.

This ASIC requires to be calibrated before use, following the procedure described in the data sheet and summarized here:
\begin{itemize}
    \item The input level of each amplifier is set just above the electronic noise produced by the detector;
    \item the TDCs and QDCs are calibrated by injecting pulses with known duration and phase, relative to the clock, from the FPGA;
    \item the dark count rate of the SiPM is measured as a function of the three thresholds, to determine the best settings to achieve an acceptable data rate and efficiency.
\end{itemize}
The first two steps are performed with the bias voltage of the SiPMs below the breakdown, while the last one at the nominal operating voltage.

The calibration is performed in an automated way and the parameters obtained from it are stored in configuration files for each DAQ board.
When data acquisition is started, these parameters are saved alongside the data, as they are needed to process the raw values of timestamp and charge associated to each hit.


\subsection{LHC signals and TTC system}
\label{subsec:lhc-signals}

The LHC clock (\SI{40.079}{MHz}, the bunch crossing frequency) and orbit (\SI{11.245}{kHz}, the revolution frequency of the LHC) signals are obtained from the Beam Synchronous Timing (BST) system, transmitted over an optical fibre using the TTC system, along with other information such as the machine mode, the beam type and energy, the GPS absolute time, etc.

A scheme of the system used in SND@LHC is shown in Figure~\ref{fig:ttc-vme-scheme}.
The BST signal is received by a dedicated board, BST-TTC, that extracts the clock and orbit signals, cleans the clock using a PLL, and distributes them to the detector using the TTC system.
The board is the same used for the read-out of the detector, described in Section~\ref{subsec:daq-electronics}, with the addition of a mezzanine card to generate the correct signal levels for the TTC modules.
%In case of absence of the BST signal, the board provides a substitute clock to the system.

The clock and synchronous commands are distributed to the DAQ boards using the TTC system, consisting of a TTCvi and a TTCex modules~\cite{ttc_web}, housed in a VME crate.
The TTCvi receives the clock and orbit signals, and generates the A-channel (trigger) and B-channel (synchronous and asynchronous commands) signals, which are encoded and transmitted by the TTCex.

The TTCvi module can be programmed and controlled using the VME bus.
A USB-to-VME converter allows it to be programmed from the server.

Variations of several nanoseconds in the phase of the clock are to be expected due to temperature changes.
For this reason, the absolute timing offset will be calibrated with the timestamps of the muons generated by $pp$ collisions in the ATLAS interaction point and detected in SND@LHC.


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/daq/ttc-vme-scheme.pdf}
    \caption{Simplified scheme of the SND@LHC TTC system.}
    \label{fig:ttc-vme-scheme}
\end{figure}

\subsection{Power supplies}
\label{subsec:psu}
The detector is powered using CAEN A2519 modules for the DAQ boards power (requiring \SI{12}{V} and \SI{2}{A} each) and A1539B modules for the bias voltage of the SiPMs (requiring up to \SI{60}{V} and up to \SI{300}{\micro A} per channel).
These modules are hosted in two SY5527 mainframes.

The control of power supplies is performed by the Detector Control system, discussed in Section~\ref{subsec:daq-dcs}, which also monitors the voltage and current draw (of both the LV and HV channels) and the presence of alarms.


\subsection{The safety and monitoring system}
\label{subsec:sms}
The Safety and Monitoring System (SMS) monitors the temperature and humidity inside the cold box, detects the presence of smoke and monitors the status of the cooling system.
It is based on the NUCLEO-H743ZI development board~\cite{nucleo_url}, featuring an ARM Cortex-M7 microcontroller.
A schematic illustration of the SMS is depicted in Figure~\ref{fig:sms}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{images/daq/SND_SMS.jpg}
    \caption{Schematic of the SMS. The items included in the dashed line are those physically installed inside the cold box.}
    \label{fig:sms}
\end{figure}

Temperature and humidity are measured in five different locations, using digital sensors (Sensirion SHT31~\cite{sensirion_trh_url}) which guarantee an accuracy of \SI{\pm 0.2}{\celsius} and \SI{\pm 2}{\percent} respectively, and a reliable I2C communication with the host microcontroller.
The positions of the sensors have been chosen to minimize the interference with the emulsion replacement procedure: three of them are positioned on the back metal plane, monitoring the temperature and humidity as close as possible to the emulsion boxes, while the remaining two sensors are placed on the opposite side, facing the cold box.
This configuration assures a comprehensive temperature and humidity mapping of the target system.

The SMS is also equipped with three smoke sensors with relay output.
They are used for fire and smoke detection and are connected to the microcontroller digital inputs with interrupt capability.

The microcontroller firmware has been developed using the Mbed OS~\cite{mbed_os_url}, an ARM Real Time Operating System.
It continuously monitors its inputs, evaluates possible alarm conditions, takes the safety actions according to the alarm levels and manages the data communication to the Detector Control System (DCS), described in Section~\ref{subsec:daq-dcs}.

The MQTT protocol~\cite{mqtt_url} is used to transmit data: the SMS system acts as a publisher for sensors data and alarm messages, which are received by the DCS, while it can receive configuration messages from the DCS.
%The system is designed to be in operation 24/7 and the frequency with which data are posted can be configured by the operator.
A watchdog has been implemented to strengthen the robustness and reliability of the system: if the microcontroller freezes for any reason, it is automatically reset by dedicated hardware.

The SMS acts as an interlock for the CAEN power supplies: if an alarm condition is detected, it can turn them off without relying on the DCS being functional.
More details about the alarm conditions are given below.

If the environmental conditions in the cold box do not meet some predefined requirements, an alarm is raised.
When an alarm occurs the SMS sends an alarm message to the MQTT broker and undertakes the needed action to secure the safety of the infrastructure according to the level of the alarm.
The control algorithm is designed to classify alarms according to three levels:

\begin{description}
    \item[Low] It occurs when the temperature or humidity readings of one sensor exceeds the set thresholds, if one smoke sensor is triggered (this is considered a low-level alarm because if only one smoke sensor is triggered, it is most likely a fault in the sensor rather than the actual presence of smoke. This assumption is based on the fact that the three smoke sensors are all inside the cold box and smoke would trigger all of them) or if the cooling system turns off.
    An alarm is posted to the broker and no further action is taken.
    \item[Medium] It occurs when the temperature or humidity readings of two or more sensors exceeds the set thresholds or if the cooling system has been turned off for more than 10 minutes.
    An alarm is posted to the broker and the power supplies are immediately turned off, to avoid the temperature inside the cold box to raise further, to protect the emulsions.
    \item[High] It occurs when two or more smoke detectors are triggered.
    An alarm is posted to the broker and the power supplies are immediately turned off. In addition, it could be setup to trigger a response of the fire brigade.
\end{description}


\subsection{Online software}
The SND@LHC online software features several components, to control different aspects of the experiment:
\begin{itemize}
    \item the Data Acquisition software, which realises the data flow from the detector to the storage;
    \item the DCS, which controls and monitors  detector services, such as  power supplies,  cooling system, etc;
    \item the LHC communication system (LHCS), which retrieves the status of the LHC beams;
    \item the Data Quality Monitor (DQM) and Real Time Analysis (RTA) system, necessary to ensure a good quality of the collected data;
    \item Logs and databases, to store the information of each run;
    \item the Experiment Control System (ECS), $i.e.$ the top-level software that controls every aspect of the detector.
\end{itemize}

A scheme of the Online software, with the different components is shown in Figure~\ref{fig:online-scheme}.
The different components are described in more details in the following sections.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/daq/online-scheme.pdf}
    \caption{Schematic drawing of the connections between different online software components.}
    \label{fig:online-scheme}
\end{figure}

\subsubsection{The Experiment Control System (ECS)}
\label{subsubsec:ecs}
The ECS is the top control level of the experiment readout system,  coordinating the software components and controlling all  data taking operations.

A hierarchical architecture is used, in which the ECS is a layer above the other online systems, preserving their autonomy to operate independently.
With this architecture, the various online programs do not strictly require the ECS to operate ($e.g$ detector calibration and data taking as a stand-alone process).

The ECS provides a unified framework to run the detector and the online systems, from which it is possible to control and to perform the data taking operation.
It also performs the logging of the relevant detector information, either in ELOG or in a database, depending on the type of information.

The ECS consists of two main software components: the ECS Process Manager (EPM) and the ECS Graphical User Interface (GUI).
The software is written in C++ and the inter-communication with the DAQ and the DCS system is done with Python scripts.

The EPM is a process which runs on the main server and acts as the communication link between  different Online system components.
It takes care of starting them and continuously monitoring their status.
The EPM process is kept alive by a cron-based watchdog: the status of the process is monitored at fixed time intervals, and restarted if it is not running. 
The EPM and its slave processes have a state machine associated with them, holding the status of the process activities.
The information of these state machines is stored in a shared memory supervised by the EPM.

The ECS GUI has been designed to ensure a simple and compact view of the run control, status of sub-detector and of the whole apparatus.
As an example, the main windows of the ECS GUI is shown in Figure~\ref{fig:ecs-gui}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/daq/ecs-gui.jpg}
    \caption{The main window of the ECS graphical interface.}
    \label{fig:ecs-gui}
\end{figure}
 

\subsubsection{Data acquisition, event building and storage}
\label{subsec:daq-events}

Each DAQ board transmits all the recorded hits to the DAQ server, where event building is performed.
The hits are grouped into events, based on their timestamp, and saved to disk as a ROOT file.

The DAQ boards also transmit periodic triggers received from the TTC system, and the DAQ server verifies that all the boards are running synchronously.
In addition, these periodic triggers are used as a hearbeat signal, to verify that all the boards are responsive, even if they are not recording data.
This process is fully controlled by the ECS, from starting  servers, to starting the data taking, sending periodic triggers, monitoring the status of each element etc.

The event building process is structured in three main steps, also shown in Figure~\ref{fig:evt-builder}:
\begin{enumerate}
    \item Hits collected by each board are grouped in ``board events'' if their timestamp is within \SI{25}{ns}. Board events contain all the hits from a given board in an event.
    \item Board events are grouped into events if their timestamp is within \SI{25}{ns}. The event timestamp corresponds to the timestamp of the earliest board event.
    \item Events are filtered and processed further, before being written to disk. The details of the processing depend on the chosen settings, but it always contains an online noise filter, described below.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/daq/daq-evt-builder.pdf}
    \caption{Schematic representation of the event builder. The colored rectangles represent queues of data being processed and the numbers identify the steps of event building, discussed in the text.}
    \label{fig:evt-builder}
\end{figure}


The noise filtering is performed in two steps:
\begin{enumerate}
    \item Events are required to have a minimum number of DAQ boards that have detected a certain number of hits. This is fast and eliminates all the events generated by a single noise hit.
    \item The hits are grouped by the plane that generated them and a more advanced requirement on the topology of the event can be imposed. This is slower, but allows for a finer control on the requirements to save an event.
\end{enumerate}

Additional data processors can be added to the software: for example, the FE calibration is applied during data acquisition.

The DAQ server writes the recorded data to a local disk and at the end of each run the data is converted in the format used by the reconstruction software and transferred to permanent storage.


\subsubsection{The Detector Control System (DCS)}
\label{subsec:daq-dcs}
The DCS controls and monitors all the detector services, namely:
\begin{itemize} 
    \item power supplies, turning them on and off, selecting  desired voltages and monitoring their status;
    \item the safety and monitoring system, discussed in Section~\ref{subsec:sms}
\end{itemize}

The voltage, currents and channel status of the power supplies are constantly monitored and transmitted to the ECS.
The ECS then acts accordingly, logging the events or raising an alarm in case of problems.

The temperature inside the cold box is constantly monitored and logged and, if it exceeds \SI{18}{\celsius}, an alarm is raised and the power to the DAQ boards is cut, to protect the emulsion films.
Alarms are also raised if a failure is detected in the cooling plant (i.e. if it turns off and stays off for more than \num{10} minuts) or if smoke is present in the cold box: in these cases the power supplies are immediately turned off.

\subsubsection{The LHC communication system}
\label{subsec:lhcs}
The LHC communication system continuously polls the status of the beam from the LHC DIP (Data Interchange Protocol) system.
The relevant information is transferred to the ECS, which can perform actions depending on them.

As an example, the ECS can automatically start the data acquisition when the LHC has stable beams, stop it when the beam is dumped and log any event that can be useful to analyse the data.

\subsubsection{The Data Quality Monitor (DQM) and Real Time Analysis (RTA) system}
\label{subsec:dqm}
The data quality monitoring is fundamental to ensure that useful data is recorded and to verify that all the sub-systems of the experiment operate correctly.

The DQM is based on a server-client pair.
The server, running on the same machine where data is being recorded, reads the written data and transmits it to the client, which, in turn, makes it available in a shared memory where several agents can read it, process it and show results in the ECS.

Several levels of complexity of the processing can be implemented: from simple hit maps, to ensure that all detector channels work as expected, to full real-time analysis, where events are fully reconstructed and a higher-level monitoring of the system can be performed (for example, a real time analysis of the detector efficiency).

==> sections/installation_old.tex <==
\section{Installation in TI18}
\label{sec:installation}

Particular effort has been paid on the studies for the integration of the needed services, to guarantee a cost efficient design of the SND detector and to evaluate the feasibility of its installation inside the TI18 cavern. The result have been a very successfully ending with a smooth installation inside TI18 and UJ18 (LHC regions) without any unexpected surprise. 

The installation was approved in the LHC Machine Committee via two Engineering change Requests \cite{ECR2021} \cite{ECRNov2021} while the infrastructure was designed based on the detailed SND Engineering specification \cite{engspec}. Is to be noted that the planing was strictly respected adapted to the LHC schedule. Any delay due to external reasons, such us the delivery of raw material, was compensated by shifting activities due to the enormous flexibility both from the CERN groups and sub-detector teams. Another challenge was the development of the construction and installation under the COVID pandemic increasing the uncertainty of the teams available and transport difficulties. Anyway, the installation have been completed with great success.

Firstly, the main infrastructure modifications and updates were performed by the CERN groups along summer 2021 completing 98\% of the activities planned up for this period. Secondly, the detector installation together with the cooling plant were put inside TI18 between November and December 2021 while the neutron shield cold box and AUG cable are to be installed in March 2022. Figure \ref{fig:integration} shows a section cut of the integration inside TI18. The neutron shielded cold box is a closed volume maintained by the evaporator at \SI{15}{\celsius} with a 45\% of relative humidity. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/Integration/IntegrationTI18.PNG}
    \caption{Detector integration in TI18}
    \label{fig:integration}
\end{figure}

The infrastructure parts and the sub-components required to operate the detector were transported on trolleys from the surface level to the LHC tunnel through the PM15 elevator (\SI{3}{\tonne} load capacity) and, then, transported along the LSS1R section of the LHC tunnel to UJ18. Two paths, over or below the LHC machine, are now available to pass equipment from the corridor side to TI18 side. The latest is located next to the footbridge and marked on the floor.

Small components can pass below the machine with a low-profile trolley limited to a \SI{37}{cm}. The dimensions were sufficient to pass the iron blocks and the target emulsions bricks, and all other smaller components. The passage will be used to pass the trolley (see Figure \ref{fig:trolley}) for the exchange of the emulsions walls.

To pass the components above the LHC machine, a rail carrying a manual hoist with a \SI{500}{\kilogram} capacity is now fixed to UJ18 ceiling. A load test was performed on site once the structure is installed. In addition, a protective structure is in place over the cryostat and cryogenic line and bolted to the floor. The vertical beams design allows full access to the quench protection box QYCDA.13R1 and cryogenic box QYCDA.13R1. The volume of the largest item to be passed is W:75\,$\times$\,H:90\,$\times$\,L:170\,cm$^3$ being the cooling plant the most demanding components in terms of size. The design of the QRL protection is a revised version of the one designed and installed in TI12 for FASER which was designed for \SI{1.3}{\tonne} falling object.

There is a clear line of sight to link the detector position with the LHC machine coordinate system. To do so, a survey fiducials positions was distributed along the detector and a geodetic network was implemented in the TI18 tunnel. 3D scanning of the area after the installation is foreseen for integration purposes. The determination of transformation parameters between the CERN Coordinate System and the local CAD system for SND in TI18 can be found in Ref. \cite{alignsystem} while the final position measurements after alignment of the base plates, target structure and muon system are collected in the Geode database \cite{Geode_database}.

\subsection{Infrastructure installation}

Several services were installed close to cryogenics and vacuum equipment and when the LHC machine was already at cryogenic temperature. In consequence, detailed procedures were followed to manage the risks associated with the proximity to to critical LHC equipment which underwent an assessment by cryogenics and safety experts concluding that all infrastructure works were carried out after removing the liquid helium and leaving the machine floating at 20K. An agreement to perform the described activities at these conditions were agreed with the TE Departmental Safety Officer. As an example, the bellows of the cryogenic distribution line and the beam position monitors feed-through were protected by a \SI{10}{\meter} aluminium thick table and protective plastic boxes, respectively, during the installation and dismantling of the scaffolding. Several activities needed the support of scaffolding to complete the works. Therefore, three scaffolding (see Figures \ref{fig:UJ18} and \ref{fig:UJ18b}) were integrated inside between the challenging environment of the UJ18 cavern. In addition, storage and assembly areas, avoiding the transport corridors, were identified. Detector components and infrastructures item were brought in batches to these areas to avoid transport bottlenecks in the access system. Figure \ref{fig:UJ18b} shows the installation and modifications within UJ18 cavern. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/Integration/uj18b.PNG}
    \caption{UJ18 prtective structure integration}
    \label{fig:UJ18b}
\end{figure}

\begin{itemize}
    \item Infrastructure updates inside UJ18 cavern:
        \begin{itemize}
            \item Installation of the protective structure as shown in Figure \ref{fig:UJ18}, including drilling fixations in the floor and the ceiling. A scan of the floor were previously done to check that any service was crossing the drilling location.
            \item Raising a section of the cable tray together with rerouting of cables to allow installing a hoist and making space for transporting over the LHC machine the largest components.
            \item Displacement of a light to make space for the installation of a rail and manual hoist above the LHC machine.
            \item Connect and route a power cable for the SND from the distribution box within UJ18 to a connection box to be installed in TI18. An 11kW power cable for the SND power supply is routed from the electrical box EVJ008/18.13R1 along the existing cable tray to be connected to the SND distribution box (EBJ1/18) within TI18.
            \item Displace of a electrical box above footbridge (EN-EL-EWS). The electrical box EOJ308/18.13R1 located above the foot bridge was moved to free the personnel passage.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/Integration/uj18a.PNG}
    \caption{UJ18 scaffolding installation}
    \label{fig:UJ18}
\end{figure}

            \item Pull the cables for AUG and lights installed in TI18. As the closest AUG is within UJ18 on the corridor side, a scaffolding was required to the cable routing over the LHC at the UJ18 IP1 end wall up to TI18. However, the emergency lights and normal lighting connections are on the TI18 side of UJ18, simplifying the connection to the LHC network.
            \item Removal of the unused \SI{40}{\meter} ventilation duct within on the TI18 side wall up to the commended door inside TI18. The three 6m long section tubes were unbolted, therefore, no cutting on site was necessary nor the installation of a SAS. The evacuation of the duct was done via point 1. Samples of the duct are to be taken to check the radiation level being bellow the clearance levels.
            \item Removal of obsolete green structure stairs to enlarge the access path towards TI18. 
            \item Barriers installation along the slope towards TI18 for safety reasons. They are fixed with two M16 anchors to the floors \cite{barriers} and their design complies with ISO 14122-3.
            \item Cable tray rerouting at the footbridge location on the TI18 due to safety reasons.
        \end{itemize}
    \item Infrastructure activities inside TI18 experimental area:
        \begin{itemize}
                \item Installation of a closed circuit cooling system and a neutron shielded cold box. A closed circuit water cooling system is required by the detector to keep the temperature of the emulsion target at \SI{15}{\celsius} in order to avoid possible fading effects and refrigerate the SciFi electronics. The cooling plant was divided in three main parts and the chillers to respect the maximum transport size over the LHC. Then, it was reassembled directly in its final place. The cooling pipes were fixed to the wall running up to the detector location. 
                \item The insulated neutron shield box is composed of an aluminium profiles skeleton and two neutron shield layers. The design includes \SI{80}{\milli\meter} squared profiles and two layers of borated polyethylene and acrylic of \SI{40}{\milli\meter} and \SI{50}{\milli\meter} thickness, respectively. The result is a \SI{1.5}{\tonne} assembly which is divided in about 200 parts of less than \SI{40}{\kilogram} installed by hand, except for the \SI{150}{\kilogram} doors which required the support of a manual hoist anchored to the cavern ceiling. The full assembly of the cold box was performed on surface inside the EHN1 building.
                \item New compressed air pipe routing. The compressed air line is connected to a T-valve of the general UJ18 line leaving a free general purpose connection.
                \item Installation of an electrical distribution box for powering the experiment and power sockets.
                \item Installation of racks for detector electronics together with its customised supports to compensate against the TI18 tunnel slope. Two 19 inch racks (XYFP01=TI18 XYFP02=TI18) are placed close to the cooling system to house the electronics of the optical fibre patch panels and SND detector. A ground distribution network was also installed and connected to the LHC ground network.
                \item Installation of a cable tray along the TI18 wall for SND cabling routing.
                \item A fire extinguisher at the entrance of the TI18 for safety requirements.
            \end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/Integration/ti18.PNG}
    \caption{TI18 services installation}
    \label{fig:TI18}
\end{figure}
    \item Inside SR1 building surface
            \begin{itemize}
                \item Installation of detector electronics for control and readout inside the rack 4Y.02-10=SR1. A new socket strip was placed inside the rack and connected to the UPS system to power the SND equipment. A label is in placed to indicated the sockets which belong to SND and FASER.   
            \end{itemize}
    \item From SR1 to TI18:
            \begin{itemize}
                \item Installation of optical fibre tubes from RE18 to TI18 over a \SI{600}{\meter} long distance. A 24SM cable including two sets of optical fibre connects the two SND racks in TI18 and the SND/FASER 4Y.02-10=SR1 rack. The optical fibre network and tubes were already in place from RE18 to SR1. Therefore, only tubes between TI18 and RE18 were installed on a low voltage cable tray close to the corridor side to easy the access. The installation of the blowing tube and fibres cable from TI18 to RE18 (rack CYFIB01=RE18) were to be carried out with the help of a rod and a ladder avoiding stepping on the LHC machine as it was at cryogenic temperature. 
             \end{itemize}

\end{itemize}

\subsection{Detector installation}

The installation of all sub-detectors inside TI18 experimental area were carried of from the 1st of November up to the 8th of December including the alignment. Later on from 1st of March 2022 to 21st the cold box fitting completed the full installation of the SND detector. The plan agreed with the LHC operation and coordination teams was closely followed up to a +/-1 day tolerance. The sequence of installation of the detector together with the neutron shield cold box and services connection was the following:

\begin{enumerate}
    \item Grouting of the base plates. The iron walls of the muon system rests on horizontal steel plates which are to be aligned by three screws with respect to IP1 nominal collision axis. The remaining space between the plate and the concrete floor was filled with grout. The grouted volume was less than \SI{0.1}{m^3}. Figure \ref{fig:TI18} shows the the grouting before the installation of the iron blocks. A wooden frame was located around each plate and the grout was poured through a \SI{80}{mm} hole located at the highest point (taking into account the slope). A cylinder-piston assembly on the hole helped to fill the full volume below the plate. The shimmed wooden frame between the plates ensured a minimum gap of \SI{25}{mm} among the first 4 plates and \SI{39}{mm} between the last small plate and the largest plate. The grout mixing was done in a bucket using an electric mixer and the TI18 was closed at the extremity with a plastic curtain to avoid spreading any dust inside the UJ18 cavern. Before any pouring the grout all plates were aligned up to a \SI{0.55}{mm} accuracy with respect to the nominal position.
    \item Iron blocks installation. The iron blocks were passed bellow the LHC machine with a low trolley and finally installed on their final position by a transportable jib crane with a total capacity of \SI{1}{\tonne}. The individual positioning precision reached was \SI{5}{mm} considering their individual maximum weight of \SI{460}{\kilogram} and means available. However, the nominal gap between walls was respected introducing a jig with the nominal separation thickness between the walls during the installation.
    \item Target and cold box feet floor marking by the survey team for a most accurate positioning of the supports. The face of the cold box base feet which is in contact with the floor is machined according to the slope tunnel. However, the target feet compensate the slope by filling the remaining space between the horizontal plate and the tunnel concrete with a resin.   
    \item Target structure assembly and refining of the walls compensators height for unloaded walls.
    \item Alignment of target unloaded mechanics by the survey team to the nominal position. The position accuracy achieved was \SI{0.5}{mm} (to be confirmed) in two of the survey fiducials having the last \SI{0.5}{mm} offset up due to a supporting food reached the extremity adjustment end. 
    \item Unloaded dummy emulsions wall as support for the later SciFi planes placement.
    \item Optical fibres patch cords and network switchers in TI18 and SR1 for the later connection of the cooling plant and SND electronics.
    \item Cooling plant, PLC and piping followed by its stand alone commissioning.
    \item Cold box feet floor and wall drilling and installation of M12 anchors for a rigid fixation of the structural frame.
    \item Detector patch panel fixation to the floor and cabling from the electronics rack to the patch panel itself. 
    \item Cabling from patch panel to SciFi and Muon system.
    \item First combined assembly among the unloaded wall boxes and SciFi inside the target structure in TI18.
    \item DAQ in TI18 and SR1 racks
    \item Grounding of the detector by the wall-fixation of two copper plates connected to the LHC ground network.
    \item Veto and muon system mechanics, detector and cabling. The planes were easily inserted among the iron walls.
    \item Muon planes alignment by the survey team. The accuracy of positioning of the planes achieved was \SI{2}{mm} setting the planes position according to the aligned target system.  
    \item Commissioning of the muon and SciFi system in parallel. To do so, a temporary connection between the SciFi and cooling plant was performed to turn on the detector. An alarm system was configured to stop the SciFi if the there is a current cut in the cooling system.
    \item Global commissioning from end of December 2021 up to the closure of the LHC at the end of March 2022.
    \item Loading of the target walls with tungsten. To do so, the SciFi is to be de-installed and the wall boxes extracted.
    \item Neutron shield cold box and evaporator. Again, SciFi and target walls are de-installed from the target structure and cables retracted to avoid any damage. A scaffolding is installed over the muon system to carry out the insertion of the neutron shield panels between the last SciFi plane and the first iron wall. The assembly inside TI18 is expected to take 1 week.
    \item SciFi and loaded wall boxes re-installation and re-commissioning of the full detector. 
    \item Target region position cross-check with the cold box in place and the loaded wall boxes. 
    \item Installation of an active wall with the first emulsion set at the very last moment before the LHC closure.  
    
\end{enumerate}

Figure \ref{fig:TI18detector} shows the different services and sub-detectors installed inside TI18.

\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{images/Integration/TI18up.PNG}
  \caption{Upstream TI18 installation}
  \label{fig:TI18up}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{images/Integration/TI18middle.PNG}
  \caption{Front view of the detector}
  \label{fig:TI18middle}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{images/Integration/TI18down.PNG}
  \caption{Side view of the detector}
  \label{fig:TI18down}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{images/Integration/TI18coldbox.PNG}
  \caption{neutron shield cold box}
  \label{fig:TI18coldbox}
\end{subfigure}
\caption{SND detector integration in TI18}
\label{fig:TI18detector}
\end{figure}


